Starting Movement Detection of Cyclists Using Smart Devices

In near future, vulnerable road users (VRUs) such as cyclists and pedestrians will be equipped with smart devices and wearables which are capable to communicate with intelligent vehicles and other traffic participants. Road users are then able to cooperate on different levels, such as in cooperative intention detection for advanced VRU protection. Smart devices can be used to detect intentions, e.g., an occluded cyclist intending to cross the road, to warn vehicles of VRUs, and prevent potential collisions. This article presents a human activity recognition approach to detect the starting movement of cyclists wearing smart devices. We propose a novel two-stage feature selection procedure using a score specialized for robust starting detection reducing the false positive detections and leading to understandable and interpretable features. The detection is modelled as a classification problem and realized by means of a machine learning classifier. We introduce an auxiliary class, that models starting movements and allows to integrate early movement indicators, i.e., body part movements indicating future behaviour. In this way we improve the robustness and reduce the detection time of the classifier. Our empirical studies with real-world data originating from experiments which involve 49 test subjects and consists of 84 starting motions show that we are able to detect the starting movements early. Our approach reaches an F1-score of 67 % within 0.33 s after the first movement of the bicycle wheel. Investigations concerning the device wearing location show that for devices worn in the trouser pocket the detector has less false detections and detects starting movements faster on average. We found that we can further improve the results when we train distinct classifiers for different wearing locations.

==> sections/method_basic_movement_forecast.tex <==






==> sections/method_first_level_mp.tex <==
\subsection{First-Level Movement Primitive Detection}
\label{subsec:movement_primitive_detection}

Slow movement primitive detection.

%The movement primitive recognition is situated in the first stage of the intention detection process. The focus of this section is on the early detection of cyclist movement types. This is realized by a classification of the 
%current movement primitive at discrete points in time with a 
%frequency of $100\,$Hz. In this work, two methods for the detection of movement primitives are realized. The first method is realized by human activity recognition techniques \cite{Bulling2014THA} based on the gyroscope and accelerometer sensory data, which is nowadays available on nearly every smartphone. The second method is based on head trajectories of the cyclist extracted from the stereo camera system at the infrastructure. In order to comply with the sampling rate of the 
%smart device, the trajectories resulting from the camera measurements are oversampled to $100\,$Hz.
%
%The gyroscope allows to detect rotating movements, such as pedaling, 
%whereas the accelerometer is better suited to detect linear movements, 
%e.g. forward movements. Furthermore, the accelerometer measurements are gravity compensated. 
%Both, the gyroscope and the linear acceleration sensor measurements are 
%rotated into the world coordinate frame using the estimated attitude of the smart device. 
%Rotational invariance is achieved by consideration of the magnitudes in geographic north and east of the rotated sensor.
%Moreover, the sensor measurements in the vertical direction are considered. 
%GPS values are not considered, since they are noisy (due to multipath effects in urban areas and even absence of signal) 
%and their sample frequency is to low to detect fast changes in the movements ($5\,$Hz) of the cyclist.
%
%Features for classification are extracted from the rotated sensor measurements, i.e. time series, using sliding window techniques. 
%A schematic of the performed steps for movement primitive detection based on smart devices and head trajectories is 
%depicted in Fig.~\ref{fig:recognition_pipeline}.
%The features extracted from the sliding windows of the smart device activity data are the mean, variance, the signals' energy~\cite{Lau2010} as well as Pearson correlations between different sensor signals in the window. Three different window lengths are considered: $0.05\,$s, $0.2\,$s and $0.5\,$s.
%Moreover, polynomial and Fourrier coefficients up to the $5$th degree are extracted~\cite{Fuchs2010}.
%Additionally, a coarse velocity estimate based on the smart devices inertial sensors is considered.
%The past velocity measurements are approximated using polynomials with orthogonal basis 
%of degree $3$ and $5$ in a sliding window manner with window length of $0.5\,$s and $2.0\,$s, respectively.
%In order to reduce the dimensionality and increase the generalization performance, a recursive feature selection procedure 
%using a linear support vector machine~\cite{Zhu2003SVM} is performed. This reduces the number of features from $147$ to $5$. 

\begin{figure} 
	\centering
	\includegraphics[width=0.6\textwidth, clip, trim=50 60 100 105]{"images/har_pipeline"}
	\caption{Process for movement primitive detection based on smart device and head trajectories.}
	\label{fig:recognition_pipeline}
	\vskip -4mm
\end{figure}

%The infrastructure-based detection of the cyclists' movement primitive is based on the cyclist's head trajectory.
%In order to achieve translational and rotational invariance, only the velocity magnitudes in the $x-y$ plane are considered.
%Additionally, the vertical component of the velocity is considered. This allows to detect the vertical head movement as an early 
%indicator of the cyclist's intention to start. Polynomials with orthogonal basis describing the shape of the trajectory are used as features.
%Three different window length $0.3\,$s, $0.5\,$s and $1.0\,$s with polynomials up to the $3$rd degree are considered. 
%The total number of $30$ features is again reduced by feature selection to $6$ essential features.
%
%Classification is done using a supervised learning techniques. Therefore, support vector machines (SVM) 
%with a radial basis function kernel are used~\cite{Bishop2006PRM}. 
%The classifier outputs probabilities, i.e. a probabilistic interpretation of the classifiers certainty. 
%%in order to be used for the forecasting models predictions. 
%Therefore, a probability calibration using a logistic sigmoid is performed~\cite{Niculescu-Mizil2005PGP}. 
%
%In order to optimize the classifier, such that it detects movement primitives as early as possible, training samples are weighted.
%This is a decay of weights toward the starting point, samples which are $0.3\,$s before the starting point are weighted less. 
%Directly after the starting point the weights are $1$ again. Additionally, a general class weight scaling is performed, 
%e.g. the starting class is assigned a higher weight. The latter weighting is only used for training of the classifier.
%The class weight parameter $cl_{w}$, the penalty term $C$, and the kernel coefficient $\gamma$ of the SVM are optimized by a grid search according to the weighted F1 score under consideration of the delay. 
%The model selection is performed as a multi-target optimization procedure trading off both criteria.

==> sections/method_overall.tex <==
\subsection{Cooperative Trajectory Forecast}
\label{sec_method_overall}
The second stage of the intention detection process is completed by the cooperative trajectory forecast. 
It is realized by a soft gating approach, weighting  
the waiting and starting forecast model in an additive fashion. A schematic of this process is depicted in Fig~\ref{fig:stage2}. 
The cooperative trajectory forecast for a particular prediction time $t_\mathrm{c}$ is formally 
defined in the following equation:

\begin{align}
y \left(t_\mathrm{c} \right) = &g \left( x_{t_\mathrm{c}}^\mathrm{w} \right) \cdot f_\mathrm{wait} \left( t_\mathrm{c}, x_{t_\mathrm{c}} \right) \\ 
&\left( 1 - g \left( x_{t_\mathrm{c}}^\mathrm{w} \right)\right) \cdot f_\mathrm{start} \left( t_\mathrm{c}, x_{t_\mathrm{c}} \right) \nonumber
\label{eq:Fusion}
\end{align}

The gating function $g$ depends on the movement primitives computed either by the smart device,
camera, or the combination of both.
It implements the model combination by weighting 
between the forecasts of the waiting and starting forecast model ($f_\mathrm{wait}$ and $f_\mathrm{start}$, 
respectively) at time $t_\mathrm{c}$. Moreover, $x_{t_\mathrm{c}}^\mathrm{w}$ denotes the input feature vector for the model fusion, whereas 
$x_{t_\mathrm{c}}$ denotes the input for the forecasting models.

The probability output generated by the movement primitive classifier (cf. Section~\ref{sec:cooperative_mp_pred}) is directly used as a gating function to weight between the predicted forecasting models. The probability is the product of the cooperative movement primitive detection. 

\begin{figure}[t]
	\includegraphics[width=0.49\textwidth,  clip, trim=0 180 370 80]{images/EnsembleForecast.pdf}
	\caption{Stage 2: Ensemble forecast approach using two models with adaptive gating function to weight the models predictions.}
	\label{fig:stage2}
	\vskip -0.3cm
\end{figure}



==> sections/method_prediction.tex <==
\subsection{Trajectory Forecast}
%\label{sec_method_cv}
The trajectory forecast of a cyclist belongs to the second stage of the intention detection process.
To forecast the future positions of the cyclist, the measured cyclist positions over the last second are transformed from 2D world coordinates into the ego coordinate system of the cyclist and are derived numerically to obtain the longitudinal and lateral velocities. The velocities are split into different temporal windows (Fig.~\ref{fig:MLP_IN_OUT}: gray segments) and are approximated with orthogonal base polynomials. The polynomial coefficients are used as input of two MLPs, one trained for waiting and one trained for starting motions. The output of the MLPs are the coefficients of polynomials, which represent the forecast longitudinal and lateral cyclist velocities over a certain forecast horizon in different temporal windows (Fig.~\ref{fig:MLP_IN_OUT}: blue segments). The velocities are reconstructed by evaluation of the coefficients, and through numerical integration of the velocities the forecast positions are retrieved. The output of both networks are combined as described in Section \ref{sec_method_overall}.

In~\cite{Zernetsch.2016} a single MLP was trained using cyclist trajectories of all motion types. For this work two networks were trained, one model for waiting ($f_\mathrm{wait}$) and one model for starting ($f_\mathrm{start}$). The reason to separate the forecast of waiting and starting motions is to reduce the forecast error, especially of starting motions. Various movements of cyclists during the waiting phase (e.g. swaying back and forth or leaning over the handlebar) lead to a decreased performance of the network described in~\cite{Zernetsch.2016} when it comes to forecasting starting motions since these movements look similar to starting, but they do not result in a large change of the cyclist velocity.

{
	\setlength{\abovecaptionskip}{5pt plus 3pt minus 3pt}
	\begin{table}[h]
%			\vskip -3mm
		\begin{center}
			\caption{Configuration of polynomials used to train the MLP.} 
			\begin{tabular}{| c | c | c | c |}
				\hline
				Polynomial & Degree & Start Time & Length \\ \hline
				$P_{in1}$ & $2$ & $-1.0\,$s & $0.5\,$s \\ \hline
				$P_{in2}$ & $3$ & $-0.5\,$s & $0.5\,$s \\ \hline
				$P_{out1}$ & $3$ & $0.0\,$s & $0.5\,$s \\ \hline
				$P_{out2}$ & $3$ & $0.5\,$s & $0.5\,$s \\ \hline
				$P_{out3}$ & $3$ & $1.0\,$s & $0.5\,$s \\ \hline
				$P_{out4}$ & $3$ & $1.5\,$s & $0.5\,$s \\ \hline
				$P_{out5}$ & $3$ & $2.0\,$s & $0.5\,$s \\ \hline
			\end{tabular}
			\label{tab:polynomials}
		\end{center}	
	
	\end{table}
}

To train the networks, 124 starting and 124 waiting scenes of uninstructed cyclists were used. The motion types were labeled manually  where the beginning of a starting motion $t_\mathrm{s}$ is defined as the first movement and the beginning of waiting $t_\mathrm{w}$ is defined as the last movement of the rear wheel of the bicycle. To train the starting network, trajectories from \mbox{$t_\mathrm{s} - 1\,$s} until the cyclists leave the field of view (FOV) were used and for the waiting network, trajectories between \mbox{$t_\mathrm{w} + 1\,$s} and \mbox{$t_\mathrm{s} - 1\,$s} were used. The networks were trained using the Resilient Backpropagation (RPROP) \cite{Riedmiller.1993} algorithm.

Tab. \ref{tab:polynomials} shows the chosen parameters for the in- and output polynomials of the MLPs. The MLP consists of two hidden layers with 20 neurons in the first and 10 neurons in the second layer. A coarse-to-fine grid search was performed, to find the optimal network structure.

\begin{figure}
	\includegraphics[width=0.5\textwidth]{images/mlp_in_output_2.png}
	\caption{Example for in- and output of MLP: cyclist head velocity (gray), current time $t_\mathrm{c} = 2.0\,$s (green), input polynomials (black), output polynomials (ochre). }
	\label{fig:MLP_IN_OUT}
\end{figure}



==> sections/method_second_level_mp.tex <==
\subsection{Second-Level Movement Primitive Detection}
\label{sec:second_level_mp_detection}
Describe movement primitive detection using HAR here.
%The MLP is optimized according to minimize the log-loss, i.e. to correctly predict the current motion primitive.
%The fusion model is optimized using adam stochastic gradient descent algorithm ({\color{magenta}reference}).

\paragraph{Human Activity Recognition Techniques}
Classifier trained using HAR goes here.

\paragraph{Convolutional Neural Network}
CNN goes here.


==> sections/results_basic_movement_first_level.tex <==
\subsection{Movement Primitive Detection}

In this section we evaluate and compare different models optimized to detect movement primitives based on smart devices, infrastructure, and cooperation.

For training and evaluation of the classifier a $5$ fold cross-validation over the test subjects is performed. Hence, 
training and test subjects are disjunctive. In order to optimize the classifiers hyperparameters, $30\%$ of each training fold are retained and used as the validation set, while the other $70\%$ are used to train the model. Hyperparameters to be optimized are $C$ and $\gamma$ of the SVM as well as the class weight $cl_{w}$ used for training.

\begin{figure}[h]
	\includegraphics[clip, trim=0 0.3cm 0 0.3cm, width=0.5\textwidth]{images/start_wait_f1_score_delay.pdf}
	\vskip 3mm
	\caption{Weighted F1 score and delay of selected models. (Green: smartphone, Magenta: head trajectory 
		and Yellow: cooperative approach.)}
	\label{fig:f1score_delay}
	\vskip -6mm
\end{figure}

Fig.~\ref{fig:f1score_delay} shows the weighted F1 score of different models plotted over the delay axis with 
various parameter settings on the test set. 
The movement primitive classifiers for smart device (S), head trajectory (H), and cooperative movement primitive classifier (C) 
are selected ($10$ models each) from the Pareto front of the weighted F1 score and delay evaluated on the validation set. 
The reported classification statistics are obtained by evaluation of the selected models on the test set 
and without consideration of the probability calibration, i.e. direct class outcome of the SVM. 
The elements of the confusion matrix plus the delay of nine selected classifiers ($3$ of each) are denoted in the last five columns of Tab~\ref{tab:motion_primitive_results}. The statistics of the confusion matrix are weighted in the same fashion as the F1 score. 

{
	\setlength{\abovecaptionskip}{5pt plus 3pt minus 3pt}
	\begin{table}[b]
		\vskip -4mm
		\begin{center}
			\caption{Classification results of selected SVM with RBF kernel according to the multi-objective parameter optimization.} 
			\resizebox{8.4cm}{!}{
			\begin{tabular}{| c | c | c | c || c | c | c | c | c | c |}
				\hline
				ID & $C$ &  $\gamma$ & $cl_{w}$ & TP & TN & FP & FN & Delay $[\text{ms}]$\\ \hline \hline
				S1 & $2^9$ & $2^{-7}$ & $22$ & $0.994$ & $0.911$ & $0.093$ & $0.006$ & $32$ \\ \hline
				S2 & $2^{-1}$ & $2^{-4}$ & $15$ & $0.996$ & $0.918$ & $0.086$ & $0.003$ & $44$ \\ \hline
				S3 & $2^{-3}$ & $2^{-4}$ & $7$ & $0.992$ & $0.940$ & $0.063$ & $0.007$ & $106$ \\ \hline \hline
				H1 & $2^{-3}$ & $2^{-7}$ & $40$ & $0.996$ & $0.906$ & $0.099$ & $0.004$ & $54$ \\ \hline
				H2 & $2^{-5}$ & $2^{-3}$ & $7$ & $0.992$ & $0.969$ & $0.033$ & $0.008$ & $222$ \\ \hline
				H3 & $2^{-1}$ & $2^{-5}$ & $5$ & $0.989$ & $0.978$ & $0.023$ & $0.011$ & $246$ \\ \hline \hline
				\textbf{C1} & $\boldsymbol{2^{-7}}$ & $\boldsymbol{2^{-3}}$ & $\boldsymbol{7}$ & $0.995$ & $0.964$ & $0.039$ & $0.004$ & $96$ \\ \hline
				C2 & $2^{-3}$ & $2^{-1}$ & $27$ & $0.994$ & $0.958$ & $0.045$ & $0.006$ & $94$ \\ \hline
				C3 & $2^{1}$ & $2^{-7}$ & $10$ & $0.992$ & $0.978$ & $0.024$ & $0.007$ & $112$ \\ \hline
			\end{tabular}}
			\label{tab:motion_primitive_results}
		\end{center}	
%		\vskip -8mm
	\end{table}
}

We observe that classifiers based on the smart device activity data have small delays but 
a high false positive rate as compared to the classifiers based on head trajectories. 
For the latter the false positive rate is lower, going 
along with a higher delay. The three classifiers $S1$ to $S3$ and $H1$ to $H3$ are representatives which range from highly sensitive with 
a high false positive rate to rather slow starting detection behavior with a low false positive rate. 
A combination of these classifiers in pairs of two are used to create the cooperative classifier as described in Sec.~\ref{sec:cooperative_mp_pred}.
The hyperparameter of the cooperative classifier are again optimized using a grid search over the parameter space.
Selected classifiers are depicted in Fig.~\ref{fig:f1score_delay} and Tab.~\ref{tab:motion_primitive_results}.
The cooperative approach trades off a low false positive rate while retaining a fast starting detection time, i.e. low delay ($<100\,$ms).
The selected cooperative classifier $C1$ for further evaluation of the trajectory forecast 
is depicted in bold in Tab.~\ref{tab:motion_primitive_results}. It is a combination of a sensitive smart device classifier $S1$, which 
reacts upon the smallest movements (e.g. first instance of beginning pedaling movement), and a conservative head trajectory classifier $H3$. It detects the starting intention after $96\,$ms with an accuracy of $90\%$ and the accuracy reaches $95\,\%$ after $212\,$ms.


==> sections/results_outline.tex <==


%In this section, we describe the evaluation of the proposed methods.

